Data Augmented 3D Semantic Scene Completion with 2D Segmentation Priors

Semantic scene completion (SSC) is a challenging Computer Vision task with many practical applications, from robotics to assistive computing. Its goal is to infer the 3D geometry in a field of view of a scene and the semantic labels of voxels, including occluded regions. In this work, we present SPAwN, a novel lightweight multimodal 3D deep CNN that seamlessly fuses structural data from the depth component of RGB-D images with semantic priors from a bimodal 2D segmentation network. A crucial difficulty in this field is the lack of fully labeled real-world 3D datasets which are large enough to train the current data-hungry deep 3D CNNs. In 2D computer vision tasks, many data augmentation strategies have been proposed to improve the generalization ability of CNNs. However those approaches cannot be directly applied to the RGB-D input and output volume of SSC solutions. In this paper, we introduce the use of a 3D data augmentation strategy that can be applied to multimodal SSC networks. We validate our contributions with a comprehensive and reproducible ablation study. Our solution consistently surpasses previous works with a similar level of complexity.

==> algo2.tex <==
\begin{algorithm}\caption{S3P Semi-supervised training}
\begin{algorithmic}
\FORALL {epochs}
    \STATE {$\mathcal D_{\textrm{labeled}}\gets \textrm{shuffle}(\mathcal D_{\textrm{labeled}}); ~i \gets 0$}
    \FORALL {$\textrm{lmb} \in \mathcal D_{\textrm{labeled}} $}
        \STATE {$P \gets \textrm{net.forward}(\textrm{lmb}); ~i \gets i + 1$}
        \STATE{$\textrm{net.backward}(L_l(\textrm{lmb},P))$}
        \IF {$i \bmod \gamma = 0$}
            \STATE {$\textrm{umb} \gets \mathcal D_{\textrm{unlabeled}}.\textrm{pull}() $}
            \STATE {$P \gets \textrm{net.forward}(\textrm{umb}) $}
            \STATE{$\textrm{net.backward}(\alpha L_u(\textrm{umb},P))$}
        \ENDIF 
    \ENDFOR
\ENDFOR   
\end{algorithmic}
    \label{alg:S3P}
\end{algorithm}


==> source_images/tables_bk.tex <==
 DCRF \cite{zhang_semantic_2018}
        &ESSC\cite{Zhang_2018_ECCV}
       &DDRNet\cite{Li_2019_CVPR}
       &TS3D\cite{Garbade_2019_CVPR_Workshops} 
      &Guedes \etal\cite{guedes_semantic_2018}
\begingroup
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table*}
  \centering
  \begin{tabular}
      { c | c c c | c c c c c c c c c c c c}
      \hline
     \multirow{ 2}{*}{model} & \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion (IoU, in percentages)} \\
   
    & prec. & rec. & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\
    \hline
    
    
    SSCNet\cite{song_semantic_2017} & 76.3 & \underline{95.2} & 73.5 & 96.3 & 84.9 & 56.8 & 28.2 & 21.3 & 56.0 & 52.7 & 33.7 & 10.9 & 44.3 & 25.4 & 46.4\\
 DCRF \cite{zhang_semantic_2018}& – & – & –& 95.4 &  84.3 &  57.7 & 24.5 &  28.2 &  63.4 & 55.3 &  34.5 &  19.6 &  45.8 &  28.7 & 48.8 \\
  VVNetR-120 \cite{guo_view-volume_2018}& 90.8 & 91.7 & 84.0 & \underline{98.4} &  87.0 &  61.0 & 54.8 &  49.3 &  83.0 & 75.5 &  55.1 &  43.5 &  68.8 &  57.7 & 66.7 \\
         EdgeNet\cite{edgnet} & \underline{93.3} & 90.6 & \underline{85.1} & 97.2 & \underline{95.3} & \underline{78.2} & 57.5 & 51.4 & 80.7 & 74.1 & 54.5 & 52.6 & 70.3 & 60.1 & 70.2\\
          ESSC\cite{Zhang_2018_ECCV} & 92.6 & 90.4 & 84.5 & 96.6 & 83.7 & 74.9 & 59.0 & 55.1 & 83.3 & 78.0 & 61.5 & 47.4 & 73.5 & 62.9 & 70.5\\%OK
       CCPNet& \textbf{98.2}&\textbf{96.8}&\textbf{91.4}&\textbf{99.2}&89.3&76.2&\underline{63.3}&\underline{58.2}&\textbf{86.1}&\textbf{82.6}&\underline{65.6}&\underline{53.2}&\underline{76.8}&\underline{65.2}&\underline{74.2}\\
       MMNet (Ours Sup)& 92.0 & 88.5 & 82.2 & 95.8 & \textbf{96.1} & \textbf{79.3} & \textbf{73.1} & \textbf{62.4} & \underline{85.6} & \underline{80.5} & \textbf{68.4} & \textbf{79.3} & \textbf{78.7} & \textbf{75.7} & \textbf{79.5} \\
\hline
    
  \end{tabular}
  \caption{\textbf{Results on SUNCG test set}. Our MMNet semantic scene completion overall results with regular supervised training surpasses by far all known previous solutions on SUNCG synthetic images.}
  \label{tab:res_suncg}
\end{table*}
\endgroup

\textbf{NYUDv2.} Table \ref{tab:res_nyu} presents the results on real images.



\begingroup
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1

\begin{table*}
  \centering
  \begin{tabular}
      { c | c | c c c | c c c c c c c c c c c c}
  \hline
      \multirow{ 2}{*}{train}&\multirow{ 2}{*}{model} & \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion (IoU, in percentages)} \\
        & & prec. & rec. & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\
  \midrule\midrule
      \multirow{10}{*}{NYU}&SSCNet\cite{song_semantic_2017} 
      & 57.0 & \textbf{94.5} & 55.1 & 15.1 & 94.7 & 24.4 & 0.0 & 12.6 & 32.1 & 35.0 & 13.0 & 7.8 & 27.1 & 10.1 & 24.7\\  %OK
       %EDGENET_EF_LR0.01_DC0.0005_13257-0.60-0.56.hdf5
       &ESSC\cite{Zhang_2018_ECCV} &  71.9  & 71.9 & 56.2 & 17.5 & 75.4 & 25.8 & 6.7 & 15.3 & 53.8 & 42.4 & 11.2 & 0.0 & 33.4 & 11.8 & 26.7\\
       %EDGENET_MF2_LR0.01_DC0.0005_71283-0.68-0.55.hdf5
       &EdgeNet\cite{edgnet} & 76.0 & 68.3 & 56.1 & 17.9 & 94.0 & 27.8 & 2.1 & 9.5 &51.8 & 44.3 & 9.4 & 3.6 & 32.5 &12.7 & 27.8\\ %OK
       &DDRNet\cite{Li_2019_CVPR} & 71.5 & 80.8 & 61.0& 21.1 & 92.1 & 33.5 & 6.8 & 14.8 & 48.3& 42.3& 13.2& 13.9& 35.3 &13.2 &30.4\\ 
       &TS3D\cite{Garbade_2019_CVPR_Workshops} & - & - & 60.0 & 9.7& 93.4& 25.5&21.0& 17.4& 55.9& 49.2& 17.0& 27.5& 39.4 &19.3 &34.1\\
       &CCPNet\cite{CCPNet}& 74.2 & \underline{90.8} &\underline{63.5} & 23.5& \textbf{96.3}& 35.7& 20.2& 25.8& 61.4& \underline{56.1}& 18.1 &28.1& 37.8& 20.1& 38.5\\
       &SketchAware\cite{Sketch}&\textbf{85.0} &81.6 &\textbf{71.3} &\textbf{43.1} &93.6 &\textbf{40.5} &24.3 &30.0 &57.1 &49.3 &\textbf{29.2} &14.3 &42.5 &\underline{28.6} &41.1\\
       &MMNet (Ours Sup.)&\underline{76.0} & 69.1 & 56.7 & 22.9 & \underline{94.8} & 35.8 & \underline{25.4} & \underline{33.2} & \underline{65.6} & 54.4 & 20.0 & \underline{33.5} & \underline{44.2} & 25.7 & \underline{41.4} \\
       &MMNet (Ours S-Sup.)&71.9 & 75.0 & 58.0 & \underline{35.6} & 94.4 & \underline{37.0} & \textbf{30.4} & \textbf{36.8} & \textbf{68.5} & \textbf{58.9} & \underline{23.4} & \textbf{32.3} & \textbf{47.9} & \textbf{30.6} & \textbf{45.1} \\
  \midrule\midrule
      \multirow{10}{*}{\makecell{SUNCG \\ +\\NYU}} &SSCNet\cite{song_semantic_2017} & 59.3 & 92.9 & 56.6 & 15.1 & 94.6 & 24.7 & 10.8 & 17.3 & 53.2 & 45.9 & 15.9 & 13.9 & 31.1 & 12.6 & 30.5\\ %OK
      &VVNetR-120\cite{guo_view-volume_2018} & 69.8 &83.1& 61.1 & 19.3 & 94.8 & 28.0 & 12.2 & 19.6 & 57.0 & 50.5 & 17.6 & 11.9 & 35.6 & 15.3 & 32.9\\ %OK
      &Guedes \etal\cite{guedes_semantic_2018} & - & - & 56.6 & - & - & - & - & - & - & - & - & - & - & - & 30.5\\
      &TNetFuse\cite{See_and_think_2018} & 67.3 & 85.8 & \textbf{60.7} & 17.3 & 92.1 & 28.0 & 16.6 & 19.3 & \textbf{57.5} & \textbf{53.8} & \textbf{17.7} & \textbf{18.5} & \textbf{38.4} & \textbf{18.9} & \textbf{34.4}\\%OK
      %EDGENET_MF2_LR0.001_DC0.0005_69521-0.67-0.57.hdf5
      &EdgeNet\cite{edgnet} & \textbf{79.1} & 66.6 & 56.7 & \textbf{22.4} & \textbf{95.0} & \textbf{29.7} & 15.5 & \textbf{20.9} & 54.1 & 53.0 & 15.6 & 14.9 & 35.0 & 14.8 & 33.7\\
     &ForkNet\cite{ForkNet}&-&-&63.4& 36.2& 93.8 &29.2 &18.9& 17.7& 61.6& 52.9 &23.3 &19.5& 45.4 &20.0 &37.1\\
      &CCPNet\cite{CCPNet} & 78.8& 94.3 &67.1& 25.5 &98.5& 38.8& 27.1 &27.3 &64.8 &58.4 &21.5 &30.1 &38.4 &23.8 &41.3\\
      &MMNet(Ours Sup) & 77.3 & 70.7 & 58.6 & 31.5 & 94.5 & 38.7 & 27.0 & 32.8 & 67.6 & 57.2 & 20.9 & 30.7 & 47.5 & 27.2 & 43.2 \\ 
        &MMNet (Ours S-Sup)&72.9 & 75.6 & 59.0 & 37.5 & 93.6 & 37.8 & 35.0 & 39.4 & 71.9 & 58.2 & 23.4 & 29.7 & 50.7 & 34.2 & 46.5 \\
      \hline
    
  \end{tabular}
  \caption{\textbf{Results on NYUDv2 test set}. Column train indicates datasets used for training the models. SUNCG + NYU means trained on SUNCG and fine tuned on NYUDv2.  Our MMNet semi-supervised and supervised models holds the best and second best overall semantic scene completion results for real world images, respectively, on both training scenarios.}
  \label{tab:res_nyu}
\end{table*}
\endgroup



==> tables/result_tables_old.tex <==

\begingroup
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table*}[ht!]
  \centering
  \begin{tabular}
            {  c | c c c | c c c c c c c c c c c c}
      \hline
     \multirow{ 2}{*}{model} & \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion (IoU, in percentages)} \\
    & prec. & rec. & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\
    \hline
    EdgeNet\cite{edgnet} & 93.3 & 90.6 & \underline{85.1}  & 97.2 & 95.3 & 78.2 & 57.5,
    & 51.4 & 80.7 & 74.1 & 54.5 & 52.6 & 70.3 &  60.1 & 70.2\\
                   ESSC\cite{Zhang_2018_ECCV} & 92.6 & 90.4 & 84.5& 96.6 & 83.7 & 74.9 & 59.0 & 55.1 & \underline{83.3} & 78.0 & 61.5 & 47.4 & 73.5 & 62.9 & 70.5\\%OK
       CCPNet\cite{CCPNet} &\textbf{98.2}&\textbf{96.8}&\textbf{91.4}&\textbf{99.2}&89.3&\underline{76.2}&\underline{63.3}&\underline{58.2}&\textbf{86.1}&\textbf{82.6}&\underline{65.6}&\underline{53.2}&\textbf{76.8}&\underline{65.2}&\underline{74.2}\\

      SISNet-BiSeNet \cite{Cai_2021_CVPR}  & 93.3 & 96.1 & 89.9 & 85.2 & 90.0 & 83.7 & 80.8 & 60.0 & 83.5 & 80.8& 68.6 & 77.3 & 86.7 & 70.1 & 78.8  \\

      SISNet-DeepLabv3 \cite{Cai_2021_CVPR}  & 92.6 & 96.3 & 89.3 & 85.4 & 90.6 & 82.6 & 80.9 & 62.9 & 84.5 &  82.6 & 71.6 & 72.6 & 85.6 & 69.7 & 79.0   \\

\hline
       \textbf{SPAwN} (ours)& 91.9 & 88.7 & 82.3 & \textbf{99.3} & \textbf{96.1} & \textbf{84.4} & \textbf{75.1} & \textbf{59.2} & 81.5 & \underline{78.1} & \textbf{67.3} & \textbf{80.1}  & \underline{76.3} & \textbf{70.4} & \textbf{78.9} \\ 
\hline
  \end{tabular}
  \caption{\textbf{Results on SUNCG test set}. Our SPAwN semantic scene completion overall results with regular supervised training surpasses by far all known previous solutions on SUNCG synthetic images.}
  \label{tab:res_suncg}
\end{table*}
\endgroup



\begingroup
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1

\begin{table*}
  \centering
  \begin{tabular}[h!]
      { c | c | c c c | c c c c c c c c c c c c}
  \hline
      \multirow{ 2}{*}{train}&\multirow{ 2}{*}{model} & \multicolumn{3}{c|}{scene completion}& \multicolumn{12}{c}{semantic scene completion (IoU, in percentages)} \\
        & & prec. & rec. & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\
  \midrule\midrule
      \multirow{4}{*}{NYUDv2}       &TS3D\cite{Garbade_2019_CVPR_Workshops}&-&-&
60.0 & 9.7& 93.4& 25.5&21.0& 17.4& 55.9& 49.2& 17.0& 27.5& 39.4 &19.3 &34.1\\
      &CCPNet\cite{CCPNet}& 74.2 & 90.8 & 63.5& 23.5& \textbf{96.3}& 35.7& 20.2& 25.8& 61.4& \underline{56.1}& 18.1 &28.1& 37.8& 20.1& 38.5\\
       &SketchAware\cite{Sketch} & 85.0 & 81.6 & 71.3 &\textbf{43.1} &93.6 &\textbf{40.5} &24.3 &30.0 &57.1 &49.3 &\textbf{29.2} &14.3 &42.5 &\underline{28.6} &41.1\\
       &\textbf{SPAwN} (ours) & 82.0 & 74.2 & 63.8 & 36.3 & 94.0 & 38.3 & 26.1 & 33.7 & 61.2 & 54.8 & 25.1 & 35.0 & 43.5 & 29.6 & 43.4 \\
  \midrule\midrule
      \multirow{4}{*}{\makecell{SUNCG \\ +\\NYUDv2}}       &TNetFuse\cite{See_and_think_2018} & 67.3 & 85.8 & 60.6& 17.3 & 92.1 & 28.0 & 16.6 & 19.3 & 57.5 & 53.8 & 17.7 & 18.5 & 38.4 & 18.9 & 34.4\\%OK
     &ForkNet\cite{ForkNet}&-&-&63.4& 36.2& 93.8 &29.2 &18.9& 17.7& 61.6& 52.9 &\underline{23.3} &19.5& \underline{45.4} &20.0 &37.1\\
      &CCPNet\cite{CCPNet}& 91.3
& 92.6 & 82.4& 25.5 &\textbf{98.5}& \textbf{38.8}& \underline{27.1} &\underline{27.3} &\underline{64.8} &\textbf{58.4} &21.5 &\underline{30.1} &38.4 &\underline{23.8} &\underline{41.3}\\

      &SISNet-BiSeNet \cite{Cai_2021_CVPR}  & 93.3 & 96.1 & 89.9 & 85.2 & 90.0 & 83.7 & 80.8 & 60.0 & 83.5 & 80.9 & 68.6 & 77.3 & 86.7 & 70.1 & 78.8  \\

      &\textbf{SPAwN} (ours)  &      81.7 & 75.7 & 64.8 & 42.9 & 93.8 & 39.7 & 27.3 & 37.2 & 66.7 & 54.9 & 28.4 & 35.1 & 47.8 & 31.5 & 45.9 \\
      \hline
  \end{tabular}
  \caption{\textbf{Results on NYUDv2 test set}. The column ``train'' indicates datasets used for training the models. SUNCG + NYU means trained on SUNCG and fine-tuned on NYUDv2.  Our SPAwN semi-supervised and supervised models hold the best and second-best overall semantic scene completion results for real-world images, on both training scenarios.}
  \label{tab:res_nyu}
\end{table*}
\endgroup


\begingroup
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1

\begin{table*}
  \centering
  \begin{tabular}[h!]
      { c | c | c c c | c c c c c c c c c c c c}
  \hline
      \multirow{ 2}{*}{train}&\multirow{ 2}{*}{model} & \multicolumn{3}{c|}{scene completion}& \multicolumn{12}{c}{semantic scene completion (IoU, in percentages)} \\
        & & prec. & rec. & IoU & ceil. & floor & wall & win. & chair & bed & sofa & table & tvs & furn. & objs. & avg. \\
  \midrule\midrule
      \multirow{3}{*}{NYUCAD}&CCPNet\cite{CCPNet} & 91.3 & 92.6 & 82.4 & 56.2& \textbf{96.6}& 58.7& \textbf{35.1}& 44.8& 68.6& 65.3& 37.6 &35.5& 53.1& 35.2& 53.2\\
       &SketchAware\cite{Sketch} & 90.6 & 92.2 & 84.2 &\textbf{59.7} &94.3 &\textbf{64.3} &32.6&51.7 &72.0 &68.7 &\underline{45.9} &19.0 &60.5 &38.5 &55.2 \\
       &\textbf{SPAwN} (ours) & 54.0 & \underline{94.7} & \underline{61.6} & 33.4 & \underline{62.8} & \underline{80.7} & \underline{68.9} & \textbf{47.6} & \textbf{41.4} & \underline{61.5} & \textbf{42.4} & \textbf{59.0} \\
  \midrule\midrule
      \multirow{3}{*}{\makecell{SUNCG \\ +\\NYUCAD}} &SSCNet\cite{song_semantic_2017}  & 59.3 & 92.9 & 56.6 & 15.1 & 94.6 & 24.7 & 10.8 & 17.3 & 53.2 & 45.9 & 15.9 & 13.9 & 31.1 & 12.6 & 30.5\\ %OK
      %EDGENET_MF2_LR0.001_DC0.0005_69521-0.67-0.57.hdf5
      &CCPNet\cite{CCPNet} & 93.4 & 91.2 & 85.1& 58.1 &\textbf{95.1}& 60.5& 36.8 &47.2 &69.3 &67.7 &39.8 &
      37.6 &55.4 &37.6 &55.0\\
      &\textbf{SPAwN} (ours)  & \underline{62.4} & \underline{94.7} & \underline{65.3} & \underline{38.3} & \textbf{70.0} & \underline{82.4} & \textbf{78.2} & \textbf{50.7} & \underline{40.2} & \textbf{64.9} & \textbf{42.4} & \underline{62.7} \\
      \hline

  \end{tabular}
  \caption{\textbf{Results on NYUDCAD}. Once again, our SPAwN semi-supervised and supervised models hold the best and second best overall semantic scene completion results on both training scenarios.}
  \label{tab:res_nyucad}
\end{table*}
\endgroup

